Scholastic: Graphical Human-Al Collaboration for Inductive and Interpretive Text Analysis

Interpretive scholars generate knowledge from text corpora by manually sampling documents, applying codes, and refining and collating codes into categories until meaningful themes emerge. Given a large corpus, machine learning could help scale this data sampling and analysis, but prior research shows that experts are generally concerned about algorithms potentially disrupting or driving interpretive scholarship. We take a human-centered design approach to addressing concerns around machine-assisted interpretive research to build Scholastic, which incorporates a machine-in-the-loop clustering algorithm to scaffold interpretive text analysis. As a scholar applies codes to documents and refines them, the resulting coding schema serves as structured metadata which constrains hierarchical document and word clusters inferred from the corpus. Interactive visualizations of these clusters can help scholars strategically sample documents further toward insights. Scholastic demonstrates how human-centered algorithm design and visualizations employing familiar metaphors can support inductive and interpretive research methodologies through interactive topic modeling and document clustering.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> future.tex <==
Engagement played a significant role in analysts' desire to use a given visualization for sampling data items. For example, P1 noted that the directory-like nature of the indented tree visualization
%, in the lack of other interesting visual features such as shape, was not as engaging as the geographical map.
lacked the engaging features that had emerged on the
% and cognitively beneficial shapes emerging in the 
Document Map. This had impacted how willing they were to sample documents with the indented tree visualization. 
% In contrast, these shapes, despite their pseudorandomness, influenced P1's sampling process. 
%the engaging nature of the document map component had been a direct precursor to P1’s sampling process. Future work should explore how depth-first sampling using word clusters could better foster curiosity about the data by combining word-level details with engaging visual features.
\rev{Future work should study how visual features upon cluster visualizations may play a role in learning and memory for qualitative data.}
% the trade-offs between 
% mental model formation, engagement, and sampling strategies that emergent geometric features may play in qualitative analysis. 


\rev{Our Discussion and Future Work sections will clarify how we intend to leverage preliminary observations about our users’ cluster exploration to inform future studies about cluster visualization. For example, even in the absence of explicit visual summaries, people were able to leverage details from the data and emergent features of the cluster’s shape to conceptualize and remember the information contained within clusters and to guide their exploration. Note that some clusters in our evaluation were pure (all data items were meat-related) while certain clusters were mixed (desserts *and* drinks). While cluster-based approaches to active learning can leverage such purities to scale expert querying, our user observations lead to interesting open questions for cluster visualization: can human experts also leverage details-on-demand about clusters to actively scale their exploration? If so, might this behavior have a capacity limit (e.g., # of clusters) or be mediated by the visualization technique used (e.g. geographical maps vs. scatterplots)? We will discuss our planned study which will evaluate the effectiveness of interactive geographical maps for memory and learning of text data.}

==> intro.tex <==
Modern social science depends heavily on the interpretation and analysis of qualitative data, such as text data from interviews, written logs, or social media archives. 
%Within positivist research, a social scientist may clean raw text metadata to include them in network models of website hyperlinks \cite{}, and within interpretivist research, they may analyze written survey responses for a Grounded Theory analysis. 
%From a positivist perspective, sociologists 
Researchers may infer statistical patterns from raw texts using topic modeling \cite{Blei2003};
% however, this positivist perspective focuses on readily quantified patterns such as word-document co-occurrences. These patterns lack grounding in the meaning of the underlying text, target research questions, and expertise of the analyst. Alternatively, 
alternatively, researchers may employ manual interpretive methods, clustering texts 
%requires a deep 
based on an in-depth reading of the data to apply codes and categories, which are then iteratively refined until meaningful themes emerge \cite{Braun2006}. The two approaches represent 
%both make 
trade-offs between efficiency and efficacy. The labor-intensive interpretive methodologies may not scale to a large corpus (e.g., large collections of online blog posts or tweets), requiring researchers to only examine (an often random) sample of texts \cite{Gauthier2022}. 
While statistical models can rapidly process a large corpus, their reliance on word-document co-occurrences or other purely statistical patterns in the absence of expert knowledge can sacrifice 
%attention to 
semantics for scale, leading to findings that may insufficiently address critical research questions \cite{Chen2018a}. 

%When presented as interactive visualizations, 
Visualizing topic models and document clusters could help interpretive scholars easily intuit the breadth of content in a text corpus 
%can serve as entry points for sampling data items from a corpus for human interpretive scholars to closely examine them, potentially leveraging the benefits of both worlds 
\cite{Baumer2020a}. 
However, our prior interview studies [removed for blind review] discovered that qualitative researchers were largely skeptic about the role of machine learning within their epistemic practices, 
% The statistical relationships defined by the model 
raising concerns about how models could bias scholars' reasoning about a corpus and drive the analysis further away from meaningful patterns otherwise hidden in the data. 
Recent visual analytics tools leverage human-AI collaborative approaches to better capture 
%statistical models 
expert knowledge and needs
%to text analysis have addressed the limitations of text models 
by incorporating human input to refine 
statistical text models \cite{El-Assady2020}.
%these clusters \cite{}  
However, these tools often focus on building better models and 
%using these tools requires the 
would require qualitative researchers to work outside of 
%the item sampling and sensemaking loops of qualitative research (
typical workflows where they iteratively apply codes to documents. 
%When removed from research questions underlying a data analysis, 
On the other hand,
% if these interactive modeling tools do not consider the research questions driving the analysis process, 
interactive models that are placed within such a workflow may benefit from clear epistemic objectives driving users to give input to the model.
% suffer from human inputs that are not 
% by clear epistemic objectives. 
%An ideal system would both assist human analysts 
We explore how visual analytics systems can instead use a machine-in-the-loop \cite{green2019disparate,green2019principles} approach to enhance established qualitative analysis workflows using statistical models, enabling researchers to surface codes and categories 
%via close 
through in-depth reading while also collecting goal-oriented user input 
%for the models. 
to refine models that scaffold, rather than replace, expert analysis.


%How the clusters should be presented for qualitative research to support information foraging is also important for incorporating models to not disrupt existing workflows by compelling users to learn novel visualization techniques. Qualitative researchers may or may not be familiar with techniques such as hierarchical node-link diagrams or treemaps for representing text clusters. On the other hand, it is much more likely that they are used to navigating topological maps or file-folder structures. When visual metaphors to such familiar tools are drawn, they may be more engaged and memorable. Engaging with these visualizations may provide a smooth entry point into data sampling, and memory for cluster structure may scaffold human curiosity where analysts are better able to keep track of where information has been sampled, and where they should sample for next.

We introduce Scholastic, a visual analytics prototype for qualitative text analysis. Scholastic builds on the strengths of interactive topic modeling and document clustering for helping organize text data at scale while minimizing disruptions to conventional qualitative analysis workflows. 
Within most qualitative text analysis methodologies, scholars first identify a document to examine and apply \textit{codes} to a passage within the document. After coding some number of documents, scholars \textit{categorize} the codes into categories (or themes \cite{Braun2006}), and continue to iteratively refine the codes and categories as they further explore the texts. Codes and categories are both meaningful units of information as well as organizational tools for re-examining relevant passages from the corpus \cite{miles2013qualitative} to further refine the coding schema.
%In our prototype tool Scholastic, w
In addition to tools for human reasoning, we consider two additional conceptualizations of codes as: 1. meaningful human input for the text model to learn from and 2. interactive filters for 
%removing information or overlays upon cluster visualizations. 
leveraging emerging knowledge to visualize the distribution of content across a large text corpus. 
In Scholastic, hierarchical document and word clusters are 
%respectively 
depicted using interactive geographical treemaps \cite{Auber2011} and indented trees \cite{Kim2020}, drawing on familiar visual metaphors while %topological maps and file-folder interfaces, and which either serve 
supporting both breadth-first and depth-first 
%entry points for sampling from a corpus. 
strategies to exploring documents within a corpus. 
%After items in a sample have been closely read, highlighted, and coded, users identify keywords within the highlighted excerpts to prepare input to the cluster models. 
% Researchers can read individual documents and highlight important passages, tagging those patterns with codes, 
%Once a researcher iterates on the codes, 
% iterating on those codes, providing metadata like keywords, and categorizing codes into a schema that the system can use to update cluster relationships based on patterns emerging from the researcher's on-going analyses.


%constrain future iterations of the cluster outputs on the analyst’s demand.

Scholastic is the result of a multi-phase co-design process with interpretive scholars, machine learning researchers, and visualization scientists. We characterized the needs for a mixed-initiative visual analytics tool to support qualitative analysis through internal discussions with experts and prior
%Throughout these 
user interviews [removed for blind review]. 
%, previously published in \cite{} and \cite{}, w
%We discovered that qualitative researchers were largely skeptic about the role of machine learning within their epistemic practices, given their goal of summarizing meaningful patterns across a corpus through human induction and interpretation. Their practices and terminologies also varied widely depending on their disciplines, but a common thread across qualitative methodologies (as is with all forms of scientific reasoning) is one of information foraging and iterative sensemaking. 
The prototype is an end-to-end tool for interactive data sampling, interactive modeling, and interpretive text analysis, executing the vision of incorporating machines
%cluster 
% algorithmic visualizations 
within the qualitative analysis workflow given a large corpus (e.g., online blog posts).
%information foraging for 
% data sampling given a large corpus (e.g., online blog posts) while deferring sensemaking to the human expert. 
We conducted a formative user study of the tool, focusing on its usability for 
corpus navigation, search, and coding processes while providing user input for the models. 
%, providing evidence that the system 
Our results indicate that \textit{Scholastic} can shift the role of AI as a collaborator for sampling data items within interpretive research methodologies, providing assistive scalability while preserving expert agency in qualitative text analysis.

% can serve as an intuitive collaborator for interpretive scholarship and demonstrates how our solution can shift the role of AI as a collaborator for sampling data items within interpretive research methodologies. 
% mixed-initiative solutions can provide assistive scalability while preserving expert agency in qualitative text analysis.


\paragraph{Contributions}
Our primary contribution is executing the vision of interactive clustering algorithms and visualizations 
%be embedded within 
supporting inductive and interpretive qualitative analysis at scale. 
%to help scale sampling data items from a large corpus, but without disruption to existing research practices. 
Toward this goal, we 
%provide the following features in our system prototype Scholastic:
make the following contributions: 

\begin{itemize}
    \item A practical characterization of the design needs for visual analytics tools supporting qualitative analysis workflows;
    \item Reading, coding, and categorization tools similar to those currently used by qualitative researchers to summarize important patterns in a text corpus;
    %with a coding schema;
    \item An interactive word and document clustering algorithm that 
    %can leverage the coding schema 
    uses the experts' codes and categories as 
    %human 
    inputs to 
    %the 
    models on-demand, adapting them to evolving knowledge; and
    %, where the coding schema inherently carry research-focused intentions behind how models should be fixed; and
    \item A visual analytics suite for an intuitive corpus navigation
    %Familiar visualization techniques for the output document and word clusters which do not require extensive sensemaking, 
    that helps scale text analysis by supporting breadth-first exploration of a corpus as well as a depth-first search for documents related to existing codes.
\end{itemize}

==> notes.tex <==
\subsection{Curiosity about cluster shapes and content}
By intentionally offering a blank map as a starting point for analysis, the geographical map did not immediately communicate quantitative summaries of their text contents.
% through labels or other conventional summary approaches. 
However, the analyst’s 
%exploration driven by 
curiosity about emergent features in the geographical map became an entry point for interpretation. Their use and interpretation of these 
% serendipitous 
features would naturally shift toward data sensemaking.
% as they steadily overlaid their own mental or conceptual models onto the clusters. 
They appeared to be able to integrate both text and shape to construct a better mental model of the space of documents \cite{tversky1991spatial},
to efficiently sample data items,
% and more effectively reason over different sets of texts for more efficient document sampling,
avoiding data items from the same cluster or to sample data items from a cluster of interest.
% as well as recall for code refinement (e.g., better able to localize specific document sets of interest). 
For P1, naming regions (e.g., ``meatopia”) provided a way to remember what documents had been sampled and to revisit similar documents later (e.g., ``maybe I should go look at what's in Meatopia”). They called the regions by names related to their shape or the document content: ``And then there's this little cell here, that's like the country on the African continent, that's like the little donut hole…”). Although P2 initially expressed confusion over some document clusters, their ability to vocalize their uncertainty (e.g., ``why does [this cluster] contain both drinks and desserts?'') also reflected curiosity-driven exploration by both verbal and spatial conceptualization of the map \cite{Dickson1988}.
% and upon being asked to recall where the drinks and dessert region was at the end of the interview, P2 was able to locate it by its shape and position. 

%For more explicit overlaying of analytical concepts, 
To add further support for document sampling, coding documents overlays 
%colored pins to depict 
landmarks on the geographical map. These landmarks enabled scholars to more actively integrate their evolving insights into their sampling strategies. For example, P2 observed how pins were still scattered across different document clusters after the model had been updated in response to their codes and categories. 
%by their coding schema. 
This context further led them to wonder 
%fostered curiosity about whether more concrete patterns 
whether the models might capture more concrete patterns 
%emerge when more codes were applied and input to the algorithm
as they continued to code. 
%On the other hand, whilst t
The indented word tree in the Code Examiner also leveraged codes and keywords to support a depth-first document sampling. However, analysts used it significantly less often. 
%of more documents, it did not have any visual features other than position and containment. This visualization was much less interacted with, and therefore did not lead to extensive engagement with the dataset. 
We hypothesize that the prescriptiveness of the word clusters (i.e., these clusters did immediately encode quantitative summaries) and the lack of unique emergent spatial features led to worries about bias and less cognitive support for an acive corpus navigation \cite{tversky1991spatial}. If so, 
%For sampling data, 
using visualization techniques that employ memorable visual features and dynamic details-on-demand as in our Document Map may help foster a range of creative user-driven sampling and code development strategies in interpretive scholarship. 
%analysts transition from exploration to data sampling and coding more effectively.

Most cluster visualizations follow the visual information-seeking mantra, starting with descriptive visual summaries of the data (overviews) that are interactively adjusted (filter, relate), and information about individual data points is available on-demand. The goal of these techniques is to better provide quantitative summaries of cluster contents at-a-glance. In contrast, our geographical map communicates only the size and hierarchical containment of each cluster: Scholastic does not impose a priori cluster keywords or filters, to avoid biasing an interpretive and inductive researcher’s attention toward any specific cluster. By design, the Document Map requires the user to demand details first, then build up their own filters and relations (i.e., codes and categories), constructing an overview through their own sensemaking process. This reversal of the information-seeking mantra allows the analyst to either implicitly develop their own mental model of a cluster’s meaning, or explicitly code documents and allow the interactive machine learning algorithm to match their outputs more closely to codes and categories identified by analysts.

\rev{Our Discussion and Future Work sections will clarify how we intend to leverage preliminary observations about our users’ cluster exploration to inform future studies about cluster visualization. For example, even in the absence of explicit visual summaries, people were able to leverage details from the data and emergent features of the cluster’s shape to conceptualize and remember the information contained within clusters and to guide their exploration. Note that some clusters in our evaluation were pure (all data items were meat-related) while certain clusters were mixed (desserts *and* drinks). While cluster-based approaches to active learning can leverage such purities to scale expert querying, our user observations lead to interesting open questions for cluster visualization: can human experts also leverage details-on-demand about clusters to actively scale their exploration? If so, might this behavior have a capacity limit (e.g., # of clusters) or be mediated by the visualization technique used (e.g. geographical maps vs. scatterplots)? We will discuss our planned study which will evaluate the effectiveness of interactive geographical maps for memory and learning of text data.}
